On Timed Scope-bounded Context-sensitive Languages

In (DLT 2016) we studied timed context sensitive languages characterized by multiple stack push down automata (MPA), with an explicit bound on number of stages where in each stage at most one stack is used (k-round MPA). In this paper, we continue our work on timed MPA and study a subclass in which a symbol corresponding to a stack being pushed in it must be popped within fixed number of contexts of that stack---scope-bounded push-down automata with multiple stacks (k-scope MPA). We use Visibly Push-down Alphabet and Event Clocks to show that timed k-scope MPA have decidable reachability problem; are closed under Boolean operations; and have an equivalent logical characterization.

==> mso.tex <==
%\section{Logical Characterization of $k$-\dtMVPA{}}
%\label{sec:mso}

%We consider a timed word  {$w = (a_1, t_1), \ldots, (a_m, t_m)$} 
Let $w = (a_1, t_1), \ldots, (a_m, t_m)$ 
be a timed word 
%{$w = (a_0, t_0), (a_1, t_1), \ldots, (a_m, t_m)$}  
over alphabet 
%$\Sigma=\langle \Sigma^i_c, \Sigma^i_{int}, \Sigma^i_r \rangle_{i=1}^n$  as a \emph{word structure} over the universe $U=\{1,2,\dots,|w|\}$ 
$\Sigma=\langle \Sigma^i_c, \Sigma^i_{l}, \Sigma^i_r \rangle_{i=1}^n$  as a \emph{word structure} over the universe $U=\{1,2,\dots,|w|\}$ 
of positions in $w$. 
We borrow definitions of predicates $Q_a(i), \ERPred{a}(i),
\EPPred{a}(i)$ from ~\cite{BDKRT15}.
% The predicates in the word structure are $Q_a(i)$ for $a \in \Sigma$ which evaluates to true at position $i$ iff \replaced[id=R3]{$w[i]=(a, \cdot)$}{$w[i]=a$}\Review{R3.B26a}, where $w[i]$ denotes the $i$th position of $w$. 
Following~\cite{lics07}, we use the matching binary relation $\mu_j(i,k)$ 
which evaluates to true iff the $i$th position is a call and the $k$th position
is its matching return corresponding to the $j$th stack. 
% We also introduce three predicates $\ERPred{a}$, $\EPPred{a}$, and $\theta_j$ capturing the following relations.
% For an interval $I$, the predicate $\ERPred{a}(i) \in I$ evaluates to true on the word structure iff $\nu^{w}_i(x_a) \in  I$ for recorder clock $x_a$. 
% For an interval $I$, the predicate $\EPPred{a}(i) \in I$ evaluates to true on the word structure iff $\nu^{w}_i(y_a) \in  I$ for predictor clock $y_a$.
We introduce the predicate $\theta_j(i) \in  I$ which evaluates to true on the
word structure  iff {$w[i] = (a, t_i)$ with $a \in \Sigma^j_r$} and {$w[i] \in \Sigma^j_r$}, and there is some $k<i$ such that 
$\mu_j(k,i)$ evaluates to true  and $t_i-t_k \in  I$.  
The predicate $\theta_j(i)$ measures time elapsed between position $k$
where a call was made on the stack $j$, and position $i$, its matching return. 
This time elapse is the age of the symbol pushed onto the stack during the call
%at position $k$. Since position $i$ is the matching return, this symbol is popped at position $i$;
at position $k$. Since position $i$ is the matching return, this
symbol is popped at $i$,
if the age lies in the interval $I$, the predicate evaluates to true.  
We define MSO($\Sigma$), the MSO logic over $\Sigma$, as:
\[
\varphi{:=}Q_a(x)~|~x {\in} X~|~\mu_j(x,y)~|~\ERPred{a}(x){\in} I~|~\EPPred{a}(x){\in}
I~|~\theta_j(x){\in} I~|\neg\varphi~|~\varphi {\vee}
\varphi|~\exists \, x.\varphi~|~\exists \, X.\varphi
\]
where $a {\in} \Sigma$, $x_a {\in} C_{\Sigma}$, $x$ is a first order variable and
$X$ is a second order variable. 

The models of a formula $\phi \in \mbox{MSO}(\Sigma)$ are timed words $w$ over
$\Sigma$. 
The semantics %of this logic  
is standard where first order variables are
interpreted over positions  of $w$ and second order variables over subsets of
positions.
We define the language $L(\varphi)$ of an MSO sentence $\varphi$ as the set of
all words satisfying $\varphi$. 
 
 
 
%Words in $Round(\Sigma,k)$, for some $k$ rounds, can be captured by an MSO formula $Bd_k(\psi)$.
%For instance if $k=1$, and $n$ stacks, the formula
%$\exists x_1. (Q_{{a}^1}(x_1) \wedge \forall y_1(y_1 \leq x_1 \rightarrow Q_{{a}^1}(y_1)) 
%\wedge \exists x_2.  (x_1 < x_2 \wedge Q_{{a}^2}(x_2) \wedge \forall
%y_2(x_1<y_2<x_2 \rightarrow Q_{{a}^2}(y_2)) \wedge  \ldots \wedge \exists x_{n}(x_{n-1} < x_{n} \wedge
%Q_{{a}^n}(x_n) \wedge last(x_n) \wedge \forall
%y_n(x_{n-1}<y_n<x_n \rightarrow Q_{{a}^n}(y_n))) ))$, 
%where ${a}^i \in \Sigma^i$ and $last(x)$ denotes $x$  is the last position,
%captures a round. This can be extended to capture $k$-round words. 
%Conjuncting the formula obtained from a \dtMVPA{} $M$ with  $Bd_k(\psi)$ accepts only those words 
%which lie in $L(M) \cap Round(\Sigma,k)$. Likewise, if one considers any MSO formula 
%$\zeta=\varphi \wedge  Bd_k(\psi)$, it can be shown that the \dtMVPA{} 
%$M$ constructed for $\zeta$ will be a $k$-\dtMVPA{}.  
% 
% 
%
 
%\ram{ 
Words in $Scope(\Sigma,k)$, for some $k$, can be captured by an MSO
%formula $Scope_k(\psi)$, given as follows.\\
formula $Scope_k(\psi)= \andover_{1 \leq j \leq n} Scope_k(\psi)^j$, where $n$ is
number of stacks, where \\
\begin{center}
$Scope_k(\psi)^j= \forall y Q_a(y) \wedge a \in \Sigma^r_j 
    \Rightarrow( \exists x\mu_j(x,y) \wedge $
$( \psi_{kcnxt}^j \wedge \psi_{matcnxt}^j \wedge
\psi_{noextracnxt} 
    ))$
\end{center}
where
$\psi_{kcnxt}^j = \exists x_1,\ldots,x_k (x_1 \leq \ldots \leq
x_k \leq y \andover_{1 \leq q \leq k} (Q_a(x_q) \wedge a \in \Sigma_j
\wedge (Q_b(x_q-1) \Rightarrow b \notin \Sigma_j))$, 
 
\noindent 
and  
$\psi_{matcnxt}^j=
\orover_{1\leq q \leq k} \forall x_i (x_q \leq x_i \leq x (Q_c(x_i)
\Rightarrow c \in \Sigma_j)) 
$, and \\
$\psi_{noextracnxt}=
\exists x_l (x_1 \leq x_l \leq y) (Q_a(l) \wedge a \in \Sigma_j \wedge
Q_b(x_{l}-1) \wedge b \in \Sigma_j) \Rightarrow x_l \in
\{x_1,\ldots,x_k\}.$ 
 
Formulas $\psi_{noextracnxt}$ and $\psi_{kcnxt}$ say that there are at most $k$
contexts of $j$-th stack, while formula $\psi_{matcnxt}$ says where 
matching call position $x$ of return position $y$ is found. 
%} 
Conjuncting the formula obtained from a \dtecmvpa{} $M$ with  $Scope(\psi)$ accepts only those words 
which lie in $L(M) \cap Scope(\Sigma,k)$. Likewise, if one considers any MSO formula 
$\zeta=\varphi \wedge  Scope(\psi)$, it can be shown that the \dtecmvpa{} 
$M$ constructed for $\zeta$ will be a $k$-\dtecmvpa{}.  
 
 
 
 
 

Hence we have the following MSO characterization. 

\begin{theorem}
\label{th:mso}
 A language $L$ over $\Sigma$ is accepted by an \name{k-scope \dtecmvpa{}} iff there is a
 MSO sentence $\varphi$ over $\Sigma$ such that $L(\varphi) \cap Scope(\Sigma,k)=L$. 
\end{theorem}

The two directions, \dtecmvpa{} 
%to MSO, as well as MSO to \dtMVPA{} can be handled using standard techniques, and can be found in Appendix \ref{app:mso}.
to MSO, as well as MSO to \dtecmvpa{} can be handled using standard
techniques, and can be found in Appendix~\ref{app:mso}.
 
% to MSO, as well as MSO to \dtMVPA{} can be handled using standard
% techniques, and is given below. 
 


 


